Predicting the Usefulness of Amazon Reviews Using Off-The-Shelf Argumentation Mining

Internet users generate content at unprecedented rates. Building intelligent systems capable of discriminating useful content within this ocean of information is thus becoming a urgent need. In this paper, we aim to predict the usefulness of Amazon reviews, and to do this we exploit features coming from an off-the-shelf argumentation mining system. We argue that the usefulness of a review, in fact, is strictly related to its argumentative content, whereas the use of an already trained system avoids the costly need of relabeling a novel dataset. Results obtained on a large publicly available corpus support this hypothesis.

==> related.tex <==
The goal of predicting the usefulness of a review, specifically an Amazon review, has already been pursued by quite a number of studies.

One of the earliest studies aims to rank Amazon reviews by their usefulness by training a regressor with a combination of different features extracted from text and metadata of the reviews, as well as features of the product~\citep{kim2006automatically}. Similar approaches employ different set of features~\cite{ngo2012analyzing}, for example including the reputation of reviewers too~\citep{baek2012helpfulness}.

Another significant work builds a customer model that describes which features of an Amazon review affect its perceived usefulness, and then it uses such features to build a regression model to predict the usefulness, expressed as the percentage of the number of people who judged a review to be useful~\citep{mudambi2010research}.

A hybrid regression model~\cite{ngo2014influence} combines text and additional features describing users (recency, frequency, monetary value) to predict the number of people who judged as useful reviews taken from Amazon and Yelp~\citep{ngo2014influence}.

To best of our knowledge, no study has explored the possibility to predict the usefulness of Amazon reviews by using or including features coming from argumentative mining.

